Physics-Informed Neural Network for Volumetric Sound field Reconstruction of Speech Signals

Recent developments in acoustic signal processing have seen the integration of deep learning methodologies, alongside the continued prominence of classical wave expansion-based approaches, particularly in sound field reconstruction. Physics-Informed Neural Networks (PINNs) have emerged as a novel framework, bridging the gap between data-driven and model-based techniques for addressing physical phenomena governed by partial differential equations. This paper introduces a PINN-based approach for the recovery of arbitrary volumetric acoustic fields. The network incorporates the wave equation to impose a regularization on signal reconstruction in the time domain. This methodology enables the network to learn the underlying physics of sound propagation and allows for the complete characterization of the sound field based on a limited set of observations. The proposed method's efficacy is validated through experiments involving speech signals in a real-world environment, considering varying numbers of available measurements. Moreover, a comparative analysis is undertaken against state-of-the-art frequency-domain and time-domain reconstruction methods from existing literature, highlighting the increased accuracy across the various measurement configurations.

==> chapters/TODO.tex <==
\begin{itemize}
    \item change notation to include functions of pressure instead of discrete representations
    \item 
\end{itemize}

==> chapters/related_work.tex <==
%! TEX root=main
\section{Related work}\label{sec:related_work}
\textcolor{red}{add this section ?}

%-------------------------------
\noindent \textbf{Kernel ridge regression with constraint of Helmholtz equation}\\
A well-known method for performing the interpolation of a function is %(quali caratteristiche deve avere questa funzione?) 
the kernel ridge regression~\cite{vovk2013kernel}, where the data points are interpolated using a positive-definite function called a reproducing kernel.
Notice that the choice of the reproducing kernel affects the properties of the desired interpolation function, since the reproducing kernel determines the function space where the solution exists. 
In the context of sound field reconstruction, authors in \cite{ueno2018kernel} proposed an interpolation problem exploiting the Kernel ridge regression method in frequency-domain.
They proved that the reproducing kernel $\kappa(\cdot)$~\cite{vovk2013kernel} given by the zero-order spherical Bessel function of the first kind~\cite{williams1999fourier} regularizes the interpolation problem to satisfy the Helmholtz equation~\eqref{eq:homHelmholtzEquation}. %, thus regularizing the problem to more accurate solutions. % recovering the sound pressure at an arbitrary position from the pressure observations.

Considering $\tilde{M}$ available microphones in position $\bm{r}_{\tilde{\mathrm{m}}}$ and $p_{\tilde{\mathrm{m}}} \in \mathbb{C}$ the frequency-domain value measured by the ${\tilde{\mathrm{m}}}^{\mathrm{th}}$ microphone at frequency $\omega$, then the interpolation problem in the kernel ridge regression frame~\cite{murphy2012machine} is formulated as an optimization problem.
The objective function to be minimized is a weighted sum of the squared residuals and the squared norm of the interpolating sound field, namely
\begin{equation}\label{eq6:interpolation_problem}
    \Hat{P}_\mathrm{opt}(\bm{r}, \omega) = \underset{\Hat{P} \in \mathbb{H}}{\arg\min} \sum_{\tilde{\mathrm{m}}\in \tilde{\mathcal{M}}}|\Hat{P}(\bm{r}_{\tilde{\mathrm{m}}}) - P_{\tilde{\mathrm{m}}}|^2 + \lambda \norm{\Hat{P}}_\mathbb{H}^2,
\end{equation}
where $\mathbb{H}$ is called \textit{reproducing kernel Hilbert space}~\cite{scholkopf2001generalized}, $\lambda \in \left.[0, \infty \right.)$ is a constant regularization parameter, and $\norm{\cdot}_\mathbb{H}$ corresponds to the total power of plane waves propagating in each direction, as described in \cite{ueno2018kernel}.

Let arrange the frequency-domain pressures $P_{\tilde{\mathrm{m}}} = P(\bm{r}_{\tilde{\mathrm{m}}}, \omega)$ in the vector
\begin{equation}
    \bm{p} = [ P_{1}, \dots,  P_{\tilde{\mathrm{m}}}]^T,
\end{equation}
where $\omega$ is omitted for notational simplicity.
Then, denoting with $\mathbf{I}_{\tilde{M}}$ the $\tilde{M} \times \tilde{M}$ identity matrix, Equation \eqref{eq6:interpolation_problem} presents a close-form solution defined as~\cite{ueno2018kernel}
\begin{equation}\label{eq6:kernel_problem}
    \Hat{P}(\bm{r})_\mathrm{opt} = \Big( (\mathbf{K} + \lambda\mathbf{I}_{\tilde{M}})^{-1}\  \bm{p} \Big)^T\ \bm{\kappa}(\bm{r}),
\end{equation}
where
\begin{equation}
    \mathbf{K} =
    \left[ {\begin{array}{ccc}
            j_0(k\norm{\bm{r}_1-\bm{r}_1}) & \cdots & j_0(k\norm{\bm{r}_1-\bm{r}_{\tilde{M}}})\\
            \vdots & \ddots & \vdots\\
            j_0(k\norm{\bm{r}_{\tilde{M}}-\bm{r}_1})  & \cdots & j_0(k\norm{\bm{r}_{\tilde{M}}-\bm{r}_{\tilde{M}}})\\
    \end{array} } \right],
\end{equation}
and
\begin{equation}\label{eq6:filter_kernel}
    \bm{\kappa}(\bm{r}) = [j_0(k\norm{\bm{r}-\bm{r}_1}), \dots, j_0(k\norm{\bm{r}-\bm{r}_{\tilde{M}}})]^T.
\end{equation}
Notice that the vector $\bm{\kappa}(\bm{r})$ represents the so-called \textit{reproducing kernels}, whose elements are defined as $\kappa(\bm{r}, \bm{r}_{\tilde{\mathrm{m}}}) = j_0(k||{\bm{r}-\bm{r}_{\tilde{\mathrm{m}}}}||)$~\cite{ueno2018kernel}, with $j_0$ the zero-order spherical Bessel function~\cite{williams1999fourier} of the first kind and $k$ the wavenumber.

It is worth noticing that the definition of the reproducing kernels $\bm{\kappa}(\bm{r})$ takes into account the physical constraint on a sound field represented by the Helmholtz equation~\eqref{eq:homHelmholtzEquation}, as demonstrated in~\cite{ueno2018kernel}.

% -------------------------	
\vspace*{5mm}
\noindent \textbf{Time-domain Equivalent Source Method}\\
In~\cite{antonello2017room}, the authors exploit the sparsity of the RIR signal in order to derive a dictionary of equivalent sources, defined as Time-domain Equivalent Source Method (TESM). 
This technique is a modified time-domain version of the ESM used to approximate the sound field in a source-free volume.
In particular, TESM is a wave-based regression method that models the pressure field as a linear combination of basis functions, thus promoting a spatio-temporal sparsity regularization~\cite{antonello2017room}.

Considering the finite set of $L$ time-domain basis functions $\phi_l(\bm{r}, t)$ weighted by the parameter $\mathsf{w}_l(t)$, we can approximate the pressure field as~\cite{costabel2004time}
\begin{equation}\label{eq6:basis_function}
    p(\bm{r}, t) \approx \sum_{l=1}^L \phi_l(\bm{r}, t) * \mathsf{w}_l(t),
\end{equation}
and the basis function employed in~\eqref{eq6:basis_function} can be well represents by Green's functions, namely~\cite{antonello2017room}
\begin{equation}\label{eq6:tesm_functions}
    \phi_l(\bm{r}, t) = \frac{1}{4\pi d_l} \delta \left( t - \frac{d_l}{c} \right),
\end{equation}
where $d_l = \norm{\bm{r}-\bm{r}_l}$ and the Dirac function $\delta(\cdot)$ is modeled as a fractional delay filter.

Authors in~\cite{antonello2017room} showed that the reconstruction of the acoustic sound field can be performed by solving the inverse relation of \eqref{eq6:basis_function} with an optimization problem.
Moreover, the unknown time domain coefficients $\mathsf{w}_l(t)$ are computed promoting a sparse solution with a $\ell_1$ norm regularization, thus increasing the performance of regularization that can be computed with minimal memory storage.

